SERPENT-VLM : Self-Refining Radiology Report Generation Using Vision Language Models

Radiology Report Generation (R2Gen) demonstrates how Multi-modal Large Language Models (MLLMs) can automate the creation of accurate and coherent radiological reports. Existing methods often hallucinate details in text-based reports that don't accurately reflect the image content. To mitigate this, we introduce a novel strategy, SERPENT-VLM (SElf Refining Radiology RePort GENeraTion using Vision Language Models), which improves the R2Gen task by integrating a self-refining mechanism into the MLLM framework. We employ a unique self-supervised loss that leverages similarity between pooled image representations and the contextual representations of the generated radiological text, alongside the standard Causal Language Modeling objective, to refine image-text representations. This allows the model to scrutinize and align the generated text through dynamic interaction between a given image and the generated text, therefore reducing hallucination and continuously enhancing nuanced report generation. SERPENT-VLM outperforms existing baselines such as LLaVA-Med, BiomedGPT, etc., achieving SoTA performance on the IU X-ray and Radiology Objects in COntext (ROCO) datasets, and also proves to be robust against noisy images. A qualitative case study emphasizes the significant advancements towards more sophisticated MLLM frameworks for R2Gen, opening paths for further research into self-supervised refinement in the medical imaging domain.

==> Chapters/Chapter3_Dataset_Collection.tex <==
% Chapter Template
\section{Dataset Description} % Main chapter title

\label{Chapter3} % Change X to a consecutive number; for 

We evaluated performance on two datasets: the widely used \textbf{IU X-Ray} benchmark \cite{iuxray_dataset} and the diverse modality \textbf{ROCO} dataset \cite{roco_dataset} for medical report generation.

The \textbf{IU X-Ray} collection is from Indiana University and is the most widely used publicly available dataset for medical report generation tasks. It contains 3,955 fully deidentified radiology reports, each associated with frontal and/or lateral chest X-rays, totaling 7,470 images. Each report has sections such as Impression, Findings, Indication, etc. We adopted the same 70/10/20 split for train/test/validation as in \cite{chen-etal-2020-generating} for fair comparison. All evaluations were on the test set.

The \textbf{ROCO} dataset on the other hand has `radiology' and `out-of-class' subsets representing 81,825 true positives and 6,127 false positives. The `out-of-class' set includes synthetic radiology images, clinical photos, portraits, compound radiology images, and digital art. For reproducibility we applied a random 80/10/10 split, giving a training set with 65,460 `radiology' and 4,902 `out-of-class' images, a validation set with 8,183 `radiology' and 612 `out-of-class' images, and a test set with 8,182 `radiology' and 613 `out-of-class' images. For consistency of experiments, we only used the `radiology' subset of images. We further carried out reports' filtering in order to remove any redundant characters in the reports.



% \begin{table}[htbp]
% \begin{center}
% \begin{tabular}{@{}lllll@{}}

% \toprule
% \textbf{Dataset} & \textbf{Train} & \textbf{Val} & \textbf{Test} & \textbf{Image Views} \\ \midrule
% IU X-Ray         & 2769           & 791          & 395           & Frontal and Lateral  \\
% ROCO             & 65460          & 8183         & 8182          & Frontal              \\ \bottomrule
% \end{tabular}
% \end{center}
% \caption{Statistics of Evaluation Datasets}
% \label{tab:dataset_stats}
% \end{table}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.7\textwidth]{images/dataset_image_final.pdf}
%     \caption{Examples of Chest X-ray report. The report lists the radiology observations regarding each area of the body examined in the imaging study.}
%     \label{fig:overview}
% \end{figure}

==> Chapters/Chapter5_Downstream_tasks.tex <==
    % Chapter Template

\section{Results And Discussion} % Main chapter title
\label{Chapter 6} 


The efficacy of the $SR^{3}GVLM$ model was rigorously evaluated against several established methods in the domain of radiology report generation and image captioning. The experiments were conducted on the IU-Xray and ROCO datasets, with the results indicating the model's superior performance.

\subsection{Quantitative Analysis}
The $SR^{3}GVLM$ model consistently outperformed other models across all evaluation metrics. Notably, on the IU-Xray dataset, it achieved the highest BLEU-4 score of 0.171 and a BertScore of 0.760, surpassing advanced models like R2GenGPT and METransformer. This indicates a significant leap in the model's ability to generate linguistically and clinically coherent reports.

\subsection{Model Performance Discussion}
The superior performance of $SR^{3}GVLM$ can be attributed to its unique integration of visual and textual information processing. The self-refining mechanism within the model proved particularly effective, enhancing the alignment of the generated reports with the visual data. This suggests that the iterative refinement process, a novel aspect of $SR^{3}GVLM$, played a crucial role in improving the accuracy and relevance of the generated reports.

\subsection{Comparison with Baseline Models}
When compared to baseline models, $SR^{3}GVLM$ demonstrated significant improvements. For instance, Show-Tell and Att2in, which employ simpler recurrent architectures and attention mechanisms, were surpassed by $SR^{3}GVLM$'s sophisticated language model and visual-text integration. Similarly, the Transformer model, known for its global attention mechanism, was outperformed by the more nuanced approach of $SR^{3}GVLM$ in capturing the intricate details of medical imaging and reports. This comparison highlights the advantage of $SR^{3}GVLM$'s advanced architecture and self-refining capabilities.





\begin{table}[htbp]
\centering
\resizebox{0.8\columnwidth}{!}{\begin{tabular}{@{}llcccccc@{}}
\toprule
\textbf{Dataset} &
  \textbf{Methods} &
  \multicolumn{1}{l}{\textbf{$Bleu_1$}} &
  \multicolumn{1}{l}{\textbf{$Bleu_2$}} &
  \multicolumn{1}{l}{\textbf{$Bleu_3$}} &
  \multicolumn{1}{l}{\textbf{$Bleu_4$}} &
  \multicolumn{1}{l}{\textbf{$Rouge_L$}} &
  \multicolumn{1}{l}{\textbf{$BertScore$}} \\ \midrule
 &
  Show-Tell &
  0.243 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.13} &
  0.108 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.078} &
  0.307 &
  0.378 \\
 &
  Att2in &
  0.248 &
  0.134 &
  0.116 &
  0.091 &
  0.309 &
  0.386 \\
 &
  AdaAtt &
  0.284 &
  0.207 &
  0.15 &
  0.126 &
  0.311 &
  0.442 \\
 &
  Transformer &
  0.372 &
  0.251 &
  0.147 &
  0.136 &
  0.317 &
  0.579 \\
 &
  M2transformer &
  0.402 &
  0.284 &
  0.168 &
  0.143 &
  0.328 &
  0.626 \\
 &
  R2Gen &
  0.47 &
  0.304 &
  0.219 &
  0.165 &
  0.371 &
  0.732 \\
 &
  R2GenCMN &
  0.475 &
  0.309 &
  0.222 &
  0.17 &
  0.375 &
  0.74 \\
 &
  MSAT &
  0.481 &
  0.316 &
  0.226 &
  0.171 &
  0.372 &
  0.749 \\
 &
  METransformer &
  0.483 &
  0.322 &
  0.228 &
  0.172 &
  0.38 &
  0.752 \\
 &
  R2GenGPT (Deep) &
  0.480 &
  0.316 &
  0.216 &
  0.169 &
  0.377 &
  0.748 \\
 &
  MiniGPT4 &
  0.494 &
  0.329 &
  0.220 &
  0.179 &
  0.390 &
  0.767 \\
 &
  BiomedGPT &
  0.516 &
  0.343 &
  0.233 &
  0.183 &
  0.403 &
  0.793 \\
 &
  LlaVA-Med &
  0.528 &
  0.346 &
  0.237 &
  0.186 &
  0.422 &
  0.845 \\
\multirow{-14}{*}{\textbf{IU-Xray}} &
  \approachName &
  \textbf{0.547} &
  \textbf{0.356} &
  \textbf{0.242} &
  \textbf{0.190} &
  \textbf{0.452} &
  \textbf{0.935} \\ \midrule
 &
  Show-Tell &
  0.104 &
  0.076 &
  0.051 &
  0.027 &
  0.089 &
  0.34 \\
 &
  Att2in &
  0.106 &
  0.077 &
  0.052 &
  0.027 &
  0.091 &
  0.347 \\
 &
  AdaAtt &
  0.122 &
  0.089 &
  0.060 &
  0.031 &
  0.104 &
  0.397 \\
 &
  Transformer &
  0.159 &
  0.116 &
  0.079 &
  0.041 &
  0.137 &
  0.521 \\
 &
  M2transformer &
  0.172 &
  0.125 &
  0.085 &
  0.044 &
  0.148 &
  0.563 \\
 &
  R2Gen &
  0.201 &
  0.147 &
  0.099 &
  0.052 &
  0.173 &
  0.658 \\
 &
  R2GenCMN &
  0.169 &
  0.148 &
  0.100 &
  0.052 &
  0.175 &
  0.665 \\
 &
  MSAT &
  0.212 &
  0.150 &
  0.102 &
  0.053 &
  0.177 &
  0.673 \\
 &
  METransformer &
  0.211 &
  0.151 &
  0.102 &
  0.053 &
  0.178 &
  0.676 \\
 &
  R2GenGPT (Deep) &
  0.213 &
  0.150 &
  0.101 &
  0.053 &
  0.177 &
  0.672 \\
 &
  MiniGPT4 &
  0.219 &
  0.156 &
  0.103 &
  0.056 &
  0.183 &
  0.689 \\
 &
  BiomedGPT &
  0.229 &
  0.163 &
  0.109 &
  0.058 &
  0.189 &
  0.712 \\
 &
  LlaVA-Med &
  0.234 &
  0.164 &
  \textbf{0.111} &
  \textbf{0.061} &
  0.198 &
  0.759 \\
\multirow{-14}{*}{\textbf{ROCO}} &
  \approachName &
  \textbf{0.243} &
  \textbf{0.169} &
  0.108 &
  0.057 &
  \textbf{0.212} &
  \textbf{0.84} \\ \bottomrule
\end{tabular}}
\caption{Results of SERPENT-VLM on Benchmark datasets}
\label{tab:results_table}
\end{table}



\begin{table}[htbp]
\centering
\resizebox{0.8\columnwidth}{!}{ \begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{Dataset} &
  \textbf{$Lambda_{Report}$} &
  \textbf{$Lambda_{Refine}$} &
  \textbf{$Bleu_1$} &
  \textbf{$Bleu_2$} &
  \textbf{$Bleu_3$} &
  \textbf{$Bleu_4$} &
  \textbf{$Rouge_L$} &
  \textbf{$BertScore$} \\ \midrule
\multirow{5}{*}{\textbf{IU-Xray}} & 0            & 1.0          & 0.416          & 0.270          & 0.184          & 0.144          & 0.344          & 0.711          \\
& \textbf{0.3} & \textbf{0.7} & \textbf{0.547} & \textbf{0.356} & \textbf{0.242} & \textbf{0.190} & \textbf{0.452} & \textbf{0.935} \\
& 0.5          & 0.5          & 0.492          & 0.320          & 0.218          & 0.171          & 0.407          & 0.842          \\
& 0.7          & 0.3          & 0.479          & 0.311          & 0.212          & 0.166          & 0.396          & 0.818          \\
& 1            & 0.0          & 0.451          & 0.311          & 0.200          & 0.157          & 0.373          & 0.771          \\ \midrule
\multirow{5}{*}{\textbf{ROCO}}    & 0            & 1            & 0.187          & 0.130          & 0.083          & 0.044          & 0.163          & 0.647          \\
  & \textbf{0.3} & \textbf{0.7} & \textbf{0.243} & \textbf{0.169} & \textbf{0.108} & \textbf{0.057} & \textbf{0.212} & \textbf{0.840} \\
  & 0.5          & 0.5          & 0.214          & 0.149          & 0.095          & 0.050          & 0.187          & 0.739          \\
  & 0.7          & 0.3          & 0.207          & 0.144          & 0.092          & 0.048          & 0.180          & 0.714          \\
  & 1            & 0            & 0.194          & 0.135          & 0.086          & 0.046          & 0.170          & 0.672          \\ \bottomrule
\end{tabular}}
\caption{Results of weight ratio changes of both the losses}
\label{tab:lambda_ratio_table}
\end{table}



\begin{table}[htbp]
\centering
\resizebox{0.8\columnwidth}{!}{\begin{tabular}{@{}llcccccc@{}}
\toprule
\textbf{Dataset} &
  \textbf{Self-Refining Loss Metric} &
  \textbf{$Bleu_1$} &
  \textbf{$Bleu_2$} &
  \textbf{$Bleu_3$} &
  \textbf{$Bleu_4$} &
  \textbf{$Rouge_L$} &
  \textbf{$BertScore$} \\ \midrule
\multirow{4}{*}{\textbf{IU-Xray}} &
  \textbf{attention based aggregation} &
  \textbf{0.547} &
  \textbf{0.356} &
  \textbf{0.242} &
  \textbf{0.190} &
  \textbf{0.452} &
  \textbf{0.935} \\
 & Average pooling                                  & 0.410 & 0.267 & 0.182 & 0.143 & 0.339 & 0.701 \\
 & top k average pooling based on attention weights & 0.465 & 0.303 & 0.206 & 0.162 & 0.384 & 0.795 \\
 & max pooling                                      & 0.383 & 0.249 & 0.169 & 0.133 & 0.316 & 0.655 \\ \midrule
\multirow{4}{*}{\textbf{ROCO}} &
  \textbf{attention based aggregation} &
  \textbf{0.243} &
  \textbf{0.169} &
  \textbf{0.108} &
  \textbf{0.057} &
  \textbf{0.212} &
  \textbf{0.840} \\
 & Average pooling                                  & 0.190 & 0.132 & 0.084 & 0.044 & 0.165 & 0.655 \\
 & top k average pooling based on attention weights & 0.199 & 0.139 & 0.089 & 0.047 & 0.174 & 0.689 \\
 & max pooling                                      & 0.170 & 0.118 & 0.076 & 0.040 & 0.148 & 0.588 \\ \bottomrule
\end{tabular}}
\caption{Results of different pooling aggregation methods}
\label{tab:aggregation technique results}
\end{table}

==> Chapters/supplementary_material.tex <==
\section{Supplementary Material}
\label{Chapter_supplementary}
\noindent\textbf{Robustness to Noisy Input Images} 

An essential aspect of our experimental evaluation was to determine the robustness of radiology report generation models to real-life image quality, which can often be low and noisy. To this end, we conducted experiments where Gaussian noise was added to radiological images before they were fed into the visual encoder. This approach aimed to simulate the varying quality of real-life medical images and assess the resilience of the models in generating accurate and comprehensive radiological reports under such conditions. We compared the performance of SERPENT-VLM, our proposed model, with two other models: LlaVA-Med \cite{li2023llavamed}, a current state-of-the-art generalistic medical model based on LLaMA-2, and BiomedGPT \cite{zhang2024biomedgpt}, a generalistic medical domain pre-trained GPT-based model.

\begin{figure}[H]
\centering
\includegraphics[width=0.8\textwidth]{images/roco_performance_metrics.png}
\caption{Performance metrics for ROCO dataset with varying levels of Gaussian noise.}
\label{fig:roco_noise}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=0.8\textwidth]{images/iu_xray_performance_metrics.png}
\caption{Performance metrics for IU-Xray dataset with varying levels of Gaussian noise.}
\label{fig:iuxray_noise}
\end{figure}

Observations from Figures \ref{fig:roco_noise} and \ref{fig:iuxray_noise} demonstrate the superior robustness and resilience of SERPENT-VLM to noisy inputs compared to LlaVA-Med and BiomedGPT. Notably, SERPENT-VLM consistently outperforms the other models across all levels of Gaussian noise variance for both datasets. For instance, in the presence of moderate noise (variance of 0.3), SERPENT-VLM maintains a higher $BLEU_1$ score, indicating its capacity to preserve the coherence and relevance of the generated reports even under degraded input conditions. This trend is consistent across other performance metrics, including $Rouge_L$ and $BertScore$, underscoring SERPENT-VLM's superior ability to extract and utilize relevant information from noisy images effectively.

Furthermore, the decline in performance metrics is less pronounced for SERPENT-VLM as the noise level increases, compared to the other models. This indicates not only the model's resilience but also its potential applicability in clinical settings, where image quality can significantly vary. Such robustness to noise is crucial for deploying automated radiology report generation systems in real-world medical settings, where they can support radiologists by providing reliable, accurate, and timely reports even when the image quality is suboptimal.

These experiments highlight the advanced capability of SERPENT-VLM in handling real-life challenges of radiological image quality, making it a promising tool for enhancing diagnostic efficiency and accuracy in the medical domain.

